Compression of Video Tracking and Bandwidth Balancing Routing in Wireless Multimedia Sensor Networks

There has been a tremendous growth in multimedia applications over wireless networks. Wireless Multimedia Sensor Networks(WMSNs) have become the premier choice in many research communities and industry. Many state-of-art applications, such as surveillance, traffic monitoring, and remote heath care are essentially video tracking and transmission in WMSNs. The transmission speed is constrained by big size of video data and fixed bandwidth allocation in constant routing path. In this paper, we present a CamShift based algorithm to compress the tracking of videos. Then we propose a bandwidth balancing strategy in which each sensor node is able to dynamically select the node for next hop with the highest potential bandwidth capacity to resume communication. Key to the strategy is that each node merely maintains two parameters that contains its historical bandwidth varying trend and then predicts its near future bandwidth capacity. Then forwarding node selects the next hop with the highest potential bandwidth capacity. Simulations demonstrate that our approach significantly increases the data received by sink node and decreases the delay on video transmission in Wireless Multimedia Sensor Network environment.

==> algorithm.tex <==
\section{Intermediate Targets Geographic Routing (ITGR)}
\label{algorithm}
In this section, we describe our routing approach. We also discuss how to merge the entries that contain pairs of 
shaded area and associated landmark. 




\subsection{Intermediate Targets Routing outline}



%Algorithm 1 shows the approaches to find  the shaded destination area when there is a hole that blocks 
%the routing path from a source node $S$ to a destination node $D$.
%We further present our intermediate targets routing algorithm. 
In ITGR routing algorithm, when a source node $S$ intends to send packets to the destination 
node $D$, it looks up its local cache to see whether $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether $D$ is in this area. If $S$ finds this kind of entry in its cache, it will consider the landmark as its 
tentative target and forward the packets to next hop. Otherwise, the  node $S$ will perform greedy or 
perimeter routing to forward  packets with destination node $D$ to next hop. 
Once the packets reach the destination, the destination  checks whether there is a landmark in the routing path or not. 
If there is, the destination will inform the source node $S$ to calculate the shaded area and then $S$ will update  
its local cache by the fresh entry $<$ $shaded\_des\_area$, $landmark$ $>$ . Hence, if node $S$ forwards packets to any nodes in
a shaded area in the future, it will
extracte the corresponding landmark node from its local cache as a tentative target and then forward packets
to next hop.




\subsection{Determining nodes located in shaded areas}

For a destination node $D$, how can we determine if it is located in a certain shaded area?
Normally, the area is enclosed by rays and partial edges of the hole polygon. 
For instance, in Fig.~\ref{fig2}, 
the area is enclosed by ray $BE$, the hole's edges from $B$ to $F$ 
and ray $FC$. While $S$ does not know node $F${'}$s$ location,
 we need to find other point as reference to evaluate if a destination node is located in the shaded area or not. 
Since no active nodes in the hole,  we can simply determine if the destination is in the area $EBPC$.
 
Suppose that points $S$,$B$ and $P${'}$s$ coordinates are $S(x_s,y_s)$,$B(x_b,y_b)$ and $P(x_p,y_p)$ respectively. 
 If a destination node $G$ satisfies the following three conditions, it must be located in the shaded area:
 \begin{enumerate}
\item $G$ and $P$ are located on the same side of line $SB$;
\item $G$ and $B$ are located on the same side of line $SP$;
\item $G$ and $S$ are located on different sides of line $BP$.
\end{enumerate} 
 
To determine it, we write line $SB${'}$s$ function as: 
\begin{displaymath}
\frac{y-y_s}{y_b-y_s}=\frac{x-x_s}{x_b-x_s}
\end{displaymath}

It can be written as: \\*
$(y_b-y_s)x-(x_b-x_s)y+(x_by_s-x_sy_b)=0$     (1)

Suppose G's coordinates are $G$$(x_g,y_g)$. To determine if $G$ is in the shaded area, 
the first step is to determine if $G$ and $P$ are in the same side of line $SB$.
We substitute $x$ and $y$ in the left term of (1) by $x_g$ and $y_g$ and derive an expression: \\*
$(y_b-y_s)x_g-(x_b-x_s)y_g+(x_by_s-x_sy_b)$    (2)


We then substitute $x$ and $y$ in the left term of (1) by $P${'}$s$ coordinates $x_p$ and $y_p$ and derive another expression: \\*
$(y_b-y_s)x_p-(x_b-x_s)y_p+(x_by_s-x_sy_b)$     (3) \\*

If the symbols of (2) and (3) are identical, $G$ and $P$ are located in the same side of line $SB$, 
we can continue to determine if $G$ is in the shaded area $T$. Otherwise, $G$ cannot be in the shaded area. 

The second step is to determine if $G$ and $B$ are located in the same side of line $SP$.We write line $SP${'}$s$ equation:\\*
$(y_p-y_s)x-(x_p-x_s)y+(x_py_s-x_sy_p)=0$     (4)\\*

Then we substitute $x$ and $y$ in the left term of (4) by $G${'}$s$ coordinates and $B${'}$s$ coordinates and derive two expressions:\\*
$(y_p-y_s)x_g-(x_p-x_s)y_g+(x_py_s-x_sy_p)$      (5)\\*
$(y_p-y_s)x_b-(x_p-x_s)y_b+(x_py_s-x_sy_p)$       (6)

 
If (5) and (6) have different symbols, $G$ cannot be in the shaded area.Otherwise, $G$ and $B$ are located in the same side of 
line $SP$. We then
write the line $BP${'}$s$ equation and substitute $G$ and $S${'}$s$ coordinates to the left term of this equation 
and then got two expressions. 
If the two expressions have different symbols, $G$ and $S$ are located in two sides of 
line $BP$. That is, $G$ is in the shaded destination area. Hence if the destination node $G$ satisfies all the three conditions 
$S$ can conclude that $G$ is located in the shaded area. 



\subsection{Entries combination}
If a node $S$ sends multiple times packets to different destinations, many entries with the 
format $<$ $shaded\_des\_area$, $landmark$ $>$ might be 
generated and be intended to be saved in the node's cache. Among these entries, some landmarks may be identical and some 
shaded destination areas may be overlapped. 
We would like to merge them to save spaces and provide efficient entry lookup in the future. So once a node $S$ sends packets to a destination 
and generates a fresh entry $<$ $area\_SUV$, $B$ $>$, 
it looks up the entries in its local cache and update them.
There are two situations $S$ needs to deal with, one is that $S$ finds an entry in its cache with the same landmark $B$ as the new generated entry. 
Another is that
$S$ finds an entry in its cache whose landmark is not $B$ but whose destination area and $area\_SUV$ are overlap each other.
%to see if 
%there is an entry with the same landmark. If there exists one, then the node updates the entry in its cache by combining the new 
%generated shaded area and the area associated with this landmark that has been saved in its cache.
In the first situation, suppose $S$ finds an entry $<$ $area\_SU^{'}V^{'}$, $B$ $>$ existing in its cache, $S$ then updates
its entries according to the following cases:\\*
Case1: $SU^{'}V^{'}$ $\subset$ $SUV$, that is: $U$ and $V$ are in different sides of $SU^{'}$,
$U$ and $V$ are in different sides of $SV^{'}$.(Fig.~\ref{fig6}) \\*
This scenario can be represented by points' coordinates as follows: Suppose 
that points $S$,$U$, $V$,$U^{'}$ and $V^{'}${'}$s$ coordinates are $S(x_s,y_s)$,$U(x_u,y_u)$, 
$V(x_v,y_v)$,$U^{'}(x_{u^{'}},y_{u^{'}})$ and $V^{'}(x_{v^{'}},y_{v^{'}})$ respectively. \\*
Then line $SU^{'}${'}$s$ equation is: \\*
$(y_{u^{'}}-y_s)x-(x_{u^{'}}-x_s)y+(x_{u^{'}}y_s-x_sy_{u^{'}})=0$  (7)\\*
We substitute $U$ and $V${'}$s$ coordinates in the left term of (7) and derive two expressions: \\*
$(y_{u^{'}}-y_s)x_u-(x_{u^{'}}-x_s)y_u+(x_{u^{'}}y_s-x_sy_{u^{'}})$  (8) \\*
$(y_{u^{'}}-y_s)x_v-(x_{u^{'}}-x_s)y_v+(x_{u^{'}}y_s-x_sy_{u^{'}})$  (9) \\*
If (8) and (9) have different symbols, then $U$ and $V$ are located in different sides of $SU^{'}$.\\*
Line $SV^{'}${'}$s$ equation is:\\*
$(y_{v^{'}}-y_s)x-(x_{v^{'}}-x_s)y+(x_{v^{'}}y_s-x_sy_{v^{'}})=0$  (10)\\*
We substitute $U$ and $V${'}$s$ coordinates in the left term of (10) and derive two expressions: \\*
$(y_{v^{'}}-y_s)x_u-(x_{v^{'}}-x_s)y_u+(x_{v^{'}}y_s-x_sy_{v^{'}})$  (11) \\*
$(y_{v^{'}}-y_s)x_v-(x_{v^{'}}-x_s)y_v+(x_{v^{'}}y_s-x_sy_{v^{'}})$  (12) \\*
If (11) and (12) have different symbols, then $U$ and $V$ are located in different sides of $SV^{'}$.\\*
The update of this scenario is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SUV$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_1.eps}
\end{center}
\caption{The case when $SU^{'}V^{'}$ $\subset$ $SUV$.}
\label{fig6}
\end{figure}





Case2: $SUV$  $\subset$ $SU^{'}V^{'}$, that is: $U^{'}$ and $V^{'}$ are in different sides of $SU$,
$U^{'}$ and $V^{'}$ are in different sides of $SV$.(Fig.~\ref{fig7}) \\* Their relative locations can still be
represented by points' coordinates as case 1.
The coresponding update is: $S$ does nothing. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_3.eps}
\end{center}
\caption{The case when $SUV$ $\subset$ $SU^{'}V^{'}$  .}
\label{fig7}
\end{figure}

Case3: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U$ and $V$ are in different sides of $SU^{'}$, 
$U$ and $V$ are in the same side of $SV^{'}$. (Fig.~\ref{fig8})
The update is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SUV^{'}$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_2.eps}
\end{center}
\caption{One case when $SUV$ and $SU^{'}V^{'}$ are overlapped. }
\label{fig8}
\end{figure}


Case4: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U^{'}$ and $V^{'}$ are in different sides of $SU$, 
$U^{'}$ and $V^{'}$ are in the same side of $SV$. (Fig.~\ref{fig9})
The update is: $S$ removes $<$ $area\_SU^{'}V^{'}$, $B$ $>$ then insert $<$ $area\_SU^{'}V$, $B$ $>$. \\*

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=8.0cm]{mer_4.eps}
\end{center}
\caption{Another case when $SUV$ and $SU^{'}V^{'}$ are overlapped. }
\label{fig9}
\end{figure}

Case5: The area of $SUV$ and $SU^{'}V^{'}$ are disjoint.The update is just to insert $<$ $area\_SUV^{'}$, $B$ $>$. \\*
In the above cases, we use the nodes' relative locations to determine two areas' inclusion relation. This method  is
avaliable for the areas caused by a hole. However, it may not avaliable for general cases of Computational Geometry.


The second situation is that  S generate a new entry 
$<$ $area\_SUV$, $B$ $>$, it looks up its local cache and 
finds an entry $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$. $area\_SUV$ and $area\_SU^{'}V^{'}$
are overlapped. For instance, in Fig.~\ref{fig10}, when $S$ sends packets to $D$, its generates an area enclosed by
$EB$, the hole perimeter from $B$ to $F$ and line $FC$(the extension of $SP$), which is represented by $SBP$ and associated with landmark $B$. When
$S$ sends packets to node $D^{'}$ later, it generates an area represented as $SB^{'}P^{'}$ and associated with landmark $B^{'}$.
A naive update is to simply insert the new generated entry to $S${'}$s$ cache. However, the new entry and the existing entry share the area
$EBF^{'}C^{'}$. Hence, if $S$ wants to send packets to a node $G$ located in the shared area, $S$ will be confused how to figure 
out the intermediate target. So we must keep all the areas stored in a certain node to be disjoint. 
In this scenario, The area $EBF^{'}C^{'}$ is associated with two landmarks $B$ and $B^{'}$,
the paths from $B$ to $G$ and from $B^{'}$ to $G$ are both greedy. The distance from  $B^{'}$ to $G$ is farer away than that from 
$B$ to $G$. We mark $B^{'}$=$argMax(distance(B,G),distance(B^{'},G))$.
We would like to let area $EBF^{'}C^{'}$ only be associated with
$B^{'}$ since if $S$ wants to send packets to a node $G$ in area $EBF^{'}C^{'}$ in the future, the tentative target $B^{'}$ will
cause less potential recursively  tentative target finding than $B$.
In general case, we mark the fresh generated entry is $<$ $area\_SUV$, $B$ $>$, $S$ looks up its entry and finds an entry $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$,
$area\_SUV$ and $area\_SU^{'}V^{'}$ are overlapped. There are four cases to update $S{'}$$s$ entries.\\*
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=7.0cm]{overlap_1.eps}
\end{center}
\caption{The case when $SUV$ and $SU^{'}V^{'}$ with different landmarks are overlapped. }
\label{fig10}
\end{figure}



Case 1: $SU^{'}V^{'}$ $\subset$ $SUV$, that is: $U$ and $V$ are in different sides of $SU^{'}$,
$U$ and $V$ are in different sides of $SV^{'}$(Fig.~\ref{fig11}). \\*
The update is: \\*
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,
$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
   inserts $<$ $area\_SUV$, $B$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$ inserts $<$ $area\_SUU^{'}$, $B$ $>$ and inserts $<$ $area\_SVV^{'}$, $B$ $>$. \\*  
$S$ does this update because once an area is the overlap of two areas, $S$ makes it be associated with the landmark that is
farer away from an arbitratry  node in the shaded common area for less recursive tentative targets finding in the future.    

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_1.eps}
\end{center}
\caption{The case when $SU^{'}V^{'}$ $\subset$ $SUV$.}
\label{fig11}
\end{figure}


Case2: $SUV$  $\subset$ $SU^{'}V^{'}$, that is: $U^{'}$ and $V^{'}$ are in different sides of $SU$,
$U^{'}$ and $V^{'}$ are in different sides of $SV$.(Fig.~\ref{fig12}) \\*
The update is:\\ If $B$ is $argMax(distance(B,G),distance(B^{'},G))$, $S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$, then
inserts $<$ $area\_SUV$, $B$ $>$, $<$ $area\_SU^{'}U$, $B^{'}$ $>$ and $<$ $area\_SV^{'}V$, $B^{'}$ $>$.\\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$, $S$ does nothing.

\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_2.eps}
\end{center}
\caption{The case when $SUV$ $\subset$ $SU^{'}V^{'}$ .}
\label{fig12}
\end{figure}


Case3: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U$ and $V$ are in different sides of $SU^{'}$, 
$U$ and $V$ are in the same side of $SV^{'}$. (Fig.~\ref{fig13})
The update is: 
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
inserts $<$ $area\_SUV$, $B$ $>$ and $<$ $area\_SVV^{'}$, $B^{'}$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,then $S$ inserts $<$ $area\_SUU^{'}$, $B$ $>$.
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_3.eps}
\end{center}
\caption{One case when $SUV$ and $SU^{'}V^{'}$ are overlapped.}
\label{fig13}
\end{figure}



Case4: The area of $SUV$ and $SU^{'}V^{'}$ are overlapped and $U^{'}$ and $V^{'}$ are in different sides of $SU$, 
$U^{'}$ and $V^{'}$ are in the same side of $SV$. (Fig.~\ref{fig14})
The update is: 
If $B$ is $argMax(distance(B,G),distance(B^{'},G))$,$S$  removes $<$ $area\_SU^{'}V^{'}$, $B^{'}$ $>$ and then
inserts $<$ $area\_SUV$, $B$ $>$ and $<$ $area\_SU^{'}U$, $B^{'}$ $>$. \\*
If $B^{'}$ is $argMax(distance(B,G),distance(B^{'},G))$,then $S$ inserts $<$ $area\_SV^{'}V$, $B$ $>$.
\begin{figure}[!htp]
\begin{center}
\includegraphics[width=4.0cm]{overope_4.eps}
\end{center}
\caption{Another case when $SUV$ and $SU^{'}V^{'}$ are overlapped.}
\label{fig14}
\end{figure}










 


\begin{comment}
\begin{algorithm}[bt] 
\begin{algorithmic}[1] 
\caption{{\em Intermediate Targets Routing}}
\label{algorithm2}
\WHILE{packets have not arrived destination D}
\STATE{$S$ looks up its local cache to see if any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and if its forwarding packets{'}$s$ destination $D^{'}$ is in the shaded destination area}
\IF{$S$ finds $D^{'}$ is in a shaded destination area in an entry}
\STATE{$S$ counts the corresponding landmark node $B$ as tentative target $D^{'}$ and forwards packets to next hop $S_1$}
\STATE{$S \leftarrow S_1$}
\ENDIF
\IF{$S$ finds no such entry}
\STATE{$S$ forwards packets with destination $D^{'}$ by GPSR to next hop $S_1$}
\STATE{$S \leftarrow S_1$}
\ENDIF
\ENDWHILE
\IF{packets arrive $D$}
\STATE{$D$ check if there the path is detour}
\IF{the path is detour}
\STATE{$D$ informs $S$ the  landmark and local minimal node $P$}
\STATE{$S$ calculates the shaded destination area and  updates its local cache}
\ENDIF
\ENDIF
\IF{the  packets never arrives the destination after a certain TTL}
\STATE{the packets are discarded and the source node reports $D$ is unreachable.}
\ENDIF


\end{algorithmic}
\end{algorithm}
\end{comment}



\subsection{ITGR routing scheme}

\begin{figure}[hbt]
\baselineskip=10.2pt

{\scriptsize
  \noindent\underline{\bf S initiates sending a packet to destination node D} \\
  \text{~~~~}Looks up its local cache to see whether any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether $D$ is in the shaded destination area; \\
  \text{~~~~}\textbf{if} finds $D$ is in a shaded destination area \\
  \text{~~~~~~~~}Counts the corresponding landmark node $B$ as tentative target $D^{'}$;\\
  \text{~~~~}forwards packets to next hop;\\
  \text{~~~~}S is waiting to receive ACK after sending the packet;\\
  \text{~~~~}\textbf{if} didn't receive an ACK after a certain TTL\\
  \text{~~~~~~~~}Reports that data sending fails;
  \\
  
  \noindent\underline{\bf When a node receives the data packet} \\
  \text{~~~~}Extracts the destination node from the packet's header; \\
  \text{~~~~}\textbf{if} this node is the destination node D\\
  \text{~~~~~~~~}Checks whether local minimal P and landmark B exists\\
  \text{~~~~~~~~}\textbf{if} they exist\\
  \text{~~~~~~~~~~~~}Sends an ACK and a $landmark\_exist\_msg$ to source containing the locations of B and P\\ 
  \text{~~~~~~~~}\textbf{else} sends an ACK to the source\\
  \text{~~~~}\textbf{else} looks up its local cache to see whether any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and whether its forwarding packets{'}$s$ destination node is in the shaded destination area; \\
  \text{~~~~~~~~}\textbf{if} finds the destination node is in a shaded destination area \\
  \text{~~~~~~~~~~~~}Counts the corresponding landmark node $B$ as tentative target $D^{'}$;\\
  \text{~~~~~~~~}Forwards packets to next hop;\\
  \\
  
  \noindent\underline{\bf When a node receives $landmark\_exist\_msg$} \\
  \text{~~~~}Calculates the shaded area by the method in Shaded Area Calculation Algorithm; \\
  \text{~~~~}Updates its local cache; \\
  
  
}

\protect\caption{Intermediate Targets Routing Algorithm}
\protect\label{routingfig}
\end{figure}







The algorithm in Fig.~\ref{routingfig} describes the routing scheme when $S$ sends packets to $D$. 
%Suppose the packets record the landmark if the path is detour then the destination will know it. 
In this algorithm, the source node
$S$ looks up its local cache to see if any $<$ $shaded\_des\_area$, $landmark$ $>$ exists 
and if its forwarding packets' destination $D$ is in the shaded destination area. If 
$S$ finds $D$ is in a shaded destination area in an entry, $S$ will count 
the corresponding landmark node $B$ as tentative target $D^{'}$  and forwards packets to next hop node, say $S_1$,
then $S_1$ will begin the entry lookup and forward packets to next hop. If $S$ finds no such entry, 
$S$ forwards packets with destination $D^{'}$ by GPSR to next hop $S_1$, $S_1$ will begin the entry lookup 
and forwrding  operations. 
%So at the beginning when $S$ attempts to forward
%packets, the $D^{'}$ in the algorithm is the final  destination node $D$. But once an entry is found, the $D^{'}$
%will be replaced  by a landmark node. 
%In any step, if the packets are forwarded to the fixed destination $D$,line 1 to line 8 will be done.
The algorithm contains two aspects, one is to select an intermediate node as tentative target to 
conduct the ITGR routing algorithm, another is to calculate the $<$ $shaded\_des\_area$, $landmark$ $>$
entry and save it to a node's cache.Both of them can be peformed  recursively.

The recursion mostly happen in the scenario such  that $\angle$ $BSD$ $\geq$ $\frac{\pi}{2}$ and
$\angle$ $BDS$ $<$ $\frac{\pi}{2}$(Fig.~\ref{fig3}) or the situation that $\angle$ $BSD$ $<$ $\frac{\pi}{2}$ 
and $\angle$ $BDS$ $\geq$ $\frac{\pi}{2}$(Fig.~\ref{fig4}). Fig.~\ref{fig5} is an instance to generate the
$<$shaded\_des\_area, landmark$>$ 
entry recursively. The first time when $S$ 
wants to send packet to $D$, it generates and saves the entry $<$ $area\_SBP$, $B$ $>$  to its cache. 
When $S$ selects $B$ as its intermediate target for routing, it will meets local minimal node $P^{'}$ and generate an entry
$<$ $area\_SB^{'}P^{'}$, $B^{'}$ $>$, then $S$ will update its cache.

\begin{figure} [!htp]
\begin{center}
\includegraphics[width=8.0cm]{figure5.eps}
%\includegraphics[width=8.0cm]{path2.eps}
%\includegraphics[width=8.0cm]{hops.eps}
\end{center}
\caption{Recursively generate shaded areas and recursively conduct ITGR}
\label{fig5}
\end{figure}

Intermediate targets routing algorithm can be recursively conducted as well. Suppose the pairs of entries 
$<$ $area\_SP^{'}P$, $B$ $>$ and $<$ $area\_SB^{'}P^{'}$, $B^{'}$ $>$ have been stored in S's local cache after updating(Fig.~\ref{fig5}). 
When S is forwarding packets whose destination is $D^{'}$,
 it looks up its local cache and finds that 
$D^{'}$  is in the shaded area $SP^{'}P$ and $B$ is the landmark,so $S$ counts $B$ it 
intermediate target. Then $S$ tries to send the packet to $B$, it looks up 
it local cache and finds node $B$ is in the shaded area $SB^{'}P^{'}$ and $B^{'}$ is the landmark, so $S$ counts 
$B^{'}$ its intermediate target, then tries to send packet to $B^{'}$ by greedy routing. Then from $B^{'}$ to $B$, 
the path is generated by greedy forwarding; 
from $B$ to $D^{'}$ , the path is greedy forwarding as well. This recursive routing makes the routing path is constructed by 
a series of sub-paths, which are all greedy forwarding paths.









